Geometric Context from Videos

We present a novel algorithm for estimating the broad 3D geometric structure of outdoor video scenes. Leveraging spatio-temporal video segmentation, we decompose a dynamic scene captured by a video into geometric classes, based on predictions made by region-classifiers that are trained on appearance and motion features. By examining the homogeneity of the prediction, we combine predictions across multiple segmentation hierarchy levels alleviating the need to determine the granularity a priori. We built a novel, extensive dataset on geometric context of video to evaluate our method, consisting of over 100 ground-truth annotated outdoor videos with over 20,000 frames. To further scale beyond this dataset, we propose a semi-supervised learning framework to expand the pool of labeled data with high confidence predictions obtained from unlabeled data. Our system produces an accurate prediction of geometric context of video achieving 96% accuracy across main geometric classes.

==> geometric_main.tex <==
\section{Geometric Context From Videos}

\noindent Our algorithm for determining geometric context from video consists of 3 main steps (\Cref{fig:flow}). First, we apply hierarchical video segmentation, obtaining spatio-temporal regions at different hierarchy levels. We rely on video segmentation to achieve (a) temporal coherence without having to explicitly enforce it in our framework and (b) by labeling regions as opposed to individual pixels we greatly reduce computational complexity. Second, we extract several features from each segment. Third, we train a classifier to discriminate segments into \emph{sky}, \emph{ground}, and \emph{vertical} classes. Additionally, a sub-classifier is trained to discriminate the vertical class further into \emph{solid}, \emph{porous}, and \emph{object}. In particular, we employ a boosted decision tree classifier with a logistic version of Adaboost~\cite{LogisticAdaboost}. We will describe each of the above steps in more detail below.

\begin{figure}[!t]
\centering
%\vspace{-0.5cm}
\includegraphics[scale=.32]{fig_flow.pdf}
\vspace*{-0.1in}
\caption{\small{Overview of our approach. First, input videos are segmented into a hierarchy of spatio-temporal regions using \cite{MatthiasSegmentation}. Then, features are extracted for each segment to train a main and sub-classifier to predict geometric context in videos.}}
\vspace*{-0.1in}
\label{fig:flow}
\end{figure}

\subsection{Video Segmentation}
\label{sec:video_segmentation}
\noindent Video segmentation aims to group similar pixels into spatio-temporal regions that are coherent in both appearance and motion. We use the hierarchical graph-based video segmentation algorithm proposed by Grundmann \etal\cite{MatthiasSegmentation,Corso2012Evaluation}, which is automatic and achieves long-term coherence. For completeness, we give a brief overview of their algorithm. Their spatio-temporal hierarchical video segmentation builds upon the graph-based image segmentation of Felzenszwalb \etal\cite{superpixel} by constructing a graph over the 3-d space-time neighbors of a voxel. This approach generates an \emph{over}-segmented video volume, which is further segmented into a hierarchy of super-regions of varying granularity. After computing region descriptors based on appearance and motion, a graph is constructed where each region from the over-segmentation forms a node and is connected to its incident regions by an edge with a weight equal to the $\chi^2$-difference of their local descriptors. This so-called region graph is used to group the over-segmented regions into super-regions by applying \cite{superpixel} to the graph. Successive application of this algorithm yields a segmentation hierarchy of the video as shown in \Cref{fig:hie} for one of our sample videos.

\begin{figure}[!t]
\centering
\includegraphics[width=0.26\columnwidth]{hier_1}
\includegraphics[width=0.26\columnwidth]{hier_2}
\includegraphics[width=0.26\columnwidth]{hier_3}
\caption{\small{Video segmentation results by applying \cite{MatthiasSegmentation}. From left to right: Hierarchy levels in increasing order; region area increases as segments from lower hierarchy levels are grouped together.}}
\vspace*{-0.15in}
\label{fig:hie}
\end{figure}

\subsection{Video Annotation}
\label{sec:annotation}
\noindent To obtain the ground truth for training and evaluation, we manually annotate over 100 videos. To greatly speed up the labeling process, we assign labels to individual spatio-temporal regions as opposed to pixels. In particular, we leverage the over-segmentation (\Cref{sec:video_segmentation}) to assign the appropriate label to each supervoxel. Though errors in the over-segmentation are limited due to the fine granularity, we need to address potential \emph{under-segmentation} errors, \ie a supervoxel contains more than one class. This is particularly of concern for the vertical class which contains a wide variety of potentially overlapping surfaces, \eg, buildings and trees, or several moving objects as cars, boats, trains, \etc. To address this problem, we introduce a new label ``mix'' to label a super-voxel, which is a mixture of two or more classes or if its identity is changing over time across geometric classes. \Cref{fig:anno_hierachy} shows the labels and their hierarchical relationship.

\begin{figure}[!h]
\centering
%\vspace{-0.1cm}
\includegraphics[scale=.28,trim=0 0 0 1cm]{fig_label_chart.pdf}
\vspace*{-0.15in}
\caption{\small{Annotation hierarchy of spatio-temporal segments: Segments are either labeled as either as a mixture of classes (mix) or assigned a main geometric class label. The vertical geometric class is further discriminated into solid, porous, and object. }}
\vspace{-0.1in}
\label{fig:anno_hierachy}
\end{figure}

To obtain a ground truth labeling for every level of the segmentation hierarchy, we leverage the ground truth labels of the over-segmented super-voxels, by pooling their labels across a super-region via majority voting (a super-region is composed of several super-voxels). Specifically, if more than 95\% of a super-region's area is assigned the same ground truth label $L$ (based on the over-segmented super-voxels it is comprised of), the super-region is assigned label $L$, otherwise it is labeled as ``mix'', as shown in \Cref{fig:anno}. We manually annotated over 20,000 frames at the over-segmentation level and then combined their labels via the above approach across the hierarchy to generate labels at higher levels. \Cref{Table:segments} gives an overview of the percentage of segments annotated for each geometric class.

\begin{figure}[!t]
\centering
%\vspace{-0.5cm}
\includegraphics[scale=0.18]{fig_anno}
\vspace*{-0.1in}
\caption{\small{Video annotation for obtaining ground truth: Over-segmented super-voxels are annotated manually. Supervoxel labels are then combined to generate ground truth for each level of segmentation hierarchy (see \Cref{sec:annotation}).% via majority voting, while accounting for possible segmentation errors by using the label ``mix'', if no label is supported by 95\% of a super-regions area.}}
}}
\vspace{-0.05in}
\label{fig:anno}
\end{figure}


%%\begin{table}[Ht]
%%\centering
%%\begin{subtable}[b]{0.45\columnwidth}
%%\small
%%\centering
%%%\begin{tabular}{|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|}\hline
%%\begin{tabular}{|c|c|c|c|}\hline
%%\emph{Sky}& 2.5\% \\\hline
%%\emph{Ground} & 15.9\%  \\\hline
%%\emph{Vertical}&  81.2\% \\\hline
%%\emph{Mix}  & 0.4\%   \\\hline
%%\end{tabular}
%%\vspace{-0.05in}
%%\caption{Main Classes}
%%\end{subtable}
%%\begin{subtable}[b]{0.45\columnwidth}
%%\small
%%%\caption{Scale inv.}
%%\centering
%%\begin{tabular}{|c|c|c|}\hline
%%%\begin{tabular}{|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|}\hline
%%\emph{Solid} & 47.5\% \\\hline
%%\emph{Porous}& 26.1\% \\\hline
%%\emph{Object}  & 7.7\%  \\\hline
%%\end{tabular}
%%\vspace{-0.05in}
%%\caption{Sub-vertical Classes}
%%\end{subtable}
%%\vspace{-0.1in}
%%\caption{\small{Percentage of segments annotated for each geometric class ($\sim2.5M$ in total at over segmented base hierarchy level).}}
%%\label{Table:segments}
%%\vspace{-0.15in}
%%\end{table}

\subsection{Features}
\label{sec:features}
\noindent We estimate the class-dependent probability of each geometric label for a segment in a frame using a wide variety of features. By segments, we refer to 2D per frame regions of the 3D spatio-temporal voxels. Specifically, we compute appearance (color, texture, location, perspective) and motion features \emph{across} each segment in a frame. %Color features provide a simple cue to identify some geometric classes, e.g., sky is usually blue or white. Texture features help identify materials and objects. A surface's position \wrt to the camera is heavily biased due to the human operator, therefore, location in the image domain provides a useful feature, \eg, sky tends to occupy the top third of a frame, with ground occupying the bottom third. 3D orientation of the scene can be incorporated into the system using the location of vanishing points and parallel line statistics building upon the method of Kosecka \textit{et al.}~\cite{VideoCompass}. 
For computing appearance features, we follow Hoeim \etal\cite{HoiemIJCV2007} and apply the publicly available code on a per-frame basis. For details please refer to \cite{HoiemIJCV2007}.

In videos, an additional feature not found in images is motion across frames. For motion features, we compute a histogram of dense optical flow (using OpenCV's implementation of Farneback's algorithm~\cite{farneback2003two}) as well as the mean motion of a segment. To capture the motion and changes in velocity and acceleration of objects across time, we compute flow histograms and mean flow for each frame $I_j$ \wrt to 3 previous frames: $I_{j-1}, I_{j-3}, I_{j-5}$. In particular, a segment $S_k$ we compute a 16-bin histogram of oriented flow vectors weighted by their corresponding magnitude. Histograms are normalized by the region area of the segment in current frame. In addition, we compute histograms for spatial flow differentials in $x$ and $y$, \ie  for the dense optical flow field $O = [O_x, O_y]$, we compute [$\partial_{x}O_x, \partial_{x}O_y]$ and $[\partial_{y}O_x, \partial_{y}O_y]$. To account for different scales, the flow differentials are computed for different kernel size of the Sobel filter (3, 5 and 7). As with the flow histograms, the spatial flow differentials are computed \wrt to 3 previous frames: $I_{j-1}, I_{j-3}, I_{j-5}$. This is similar to the approach of \cite{dalal2006flow}, which has been shown to to be helpful to the task of object detection in videos. \Cref{Table:feat} lists all of our motion based features used for estimating geometric context of video. 

\begin{table}[!h]
\centering
\small
\begin{tabular}{|c l|}
  \hline
  \multicolumn{2}{|c|}{\textbf{Motion based Features}} \\
  \hline
  \textbf{Dimensions} & \textbf{Description} \\
  $16\times3$ & Histogram of dense optical flow O of \\
	  &reference frame $I_j$ \wrt $I_{j-1}, I_{j-3}, I_{j-5}$.\\
  $16\times2\times3\times3$ & Histogram of differential of dense \\
	  &optical flow O in x and y, \\
	  & \ie [$\partial_{x}O_x, \partial_{x}O_y]$ and $[\partial_{y}O_x, \partial_{y}O_y$], across\\
	  & 3 kernel sizes of differential (3, 5, and 7) \\
	  & for reference frame $I_j$ \wrt $I_{j-1}, I_{j-3}, I_{j-5}$.\\
  $2\times3$ & Mean flow of a segment minus min. mean\\
  &  flow across all segments of current frame.\\
  $2\times3$ & Mean location change in x and y \\
  & for reference frame $I_j$ \wrt $I_{j-1}, I_{j-3}, I_{j-5}$.\\
  $2 \times 2 \times 3$ & 10th and 90th percentile of location change\\
  	& in x and y for frame $I_j$  \wrt $I_{j-3}, I_{j-5}$.\\\
  $1 \times 3$ & Magnitude of location change of mean,\\
  	& 10th and 90th percentile. \\  
  \hline
\end{tabular}
\vspace{-0.1in}
\caption{\small{List of flow and motion based features computed per frame $I_j$ and per segment $S_k$. See text for details. Appearance features are adopted using the approach of Hoeim \etal~\cite{HoiemIJCV2007}.}}
\label{Table:feat}
\vspace{-0.3in}
\end{table}

\subsection{Multiple Segmentations}
\noindent As the appropriate granularity of the segmentation is not known a priori, we make use of multiple segmentations across several hierarchy levels, utilizing the increased spatial support of the segments at higher levels to compute features. In particular, we combine the individually predicted labels based on homogeneity of the segments. Homogeneity is defined in our case as the probability of the segment \emph{not} being a mixture of several classes, \ie \emph{not} having the label mix (for details, see \Cref{sec:classification}). We generate multiple segmentations of the scene at various granularity levels ranging from 10\% to 50\% of the hierarchy height using \cite{MatthiasSegmentation} in increments of 10\% (5 hierarchy levels in total).

\begin{figure*}
\centering
%\vspace{-0.5cm}
\includegraphics[width=0.7\textwidth]{fig_confidence2.pdf}
\vspace{-0.1in}
\caption{\small{Input video image, predicted labels and confidence for each geometric class. Notice, that trees are correctly assigned high probability for porous class, walls for solid class, and humans and cars have high confidence for the object class.}}
\vspace{-0.1in}
\label{fig:vert_conf}
\end{figure*}

\subsection{Classification}
\label{sec:classification}
\noindent We evaluate our method using boosted decision trees based on a logistic regression version of Adaboost~\cite{LogisticAdaboost} that outputs the class probability for each segment in a frame and perform 5-fold cross validation. We train two multi-class classifiers to predict the geometric labels, first to discriminate among the main classes (sky, ground, and vertical), and second for further sub-classification of vertical class (buildings, porous, and objects). In addition to the two multi-class classifiers, we independently train a homogeneity classifier that estimates the probability of the segment being a single label segment or part of the class ``mix''. We refer to this probability as the \emph{homogeneity} of a segment. This will enables us to take advantage of multiple segmentations, by combining the label confidence of segments based on their homogeneity. We combine the predictions of all three classifiers probabilistically to estimate the final label as described below.
\vspace*{-0.3in}
\paragraph{Training:} We extract the features described in \Cref{sec:features} from each segment of a training video. As the segments vary across time, we opt to extract features for each frame for the same segment to provide discriminating information over time (\eg appearance, motion, and pose of objects) as opposed to sampling features from unique spatio-temporal regions only. In addition, features are extracted independently for different hierarchical segmentation levels to provide instances with more spatial support. We extract features from 5 segmentation hierarchical levels ranging from 10\% to 50\% of the hierarchy height. Segments with a single ground truth label are used to train main and sub-vertical classifiers. We train the homogeneity classifier by providing examples of a single label and ``mix'' label segments as positive and negative instances.
\vspace*{-0.15in}
\paragraph{Prediction:} To predict the labels for a test video, features are extracted from each segment. A spatio-temporal region is labeled on a per-frame basis with the final classification being obtained by averaging the predicted class-posteriors across frames. We label main and sub-vertical geometrical classes independently, \ie we compute the sub-vertical labels for all the segments in a frame but only apply it to segments labeled as vertical by main classifier.

When using multiple segmentations across different hierarchies, a super-pixel is part of different segments at each level of segmentation hierarchy. To determine the label $y_i$ of \emph{super-pixel} $i$, class-posteriors from all segments in the hierarchy $s_j$, containing the super-pixel are combined using a weighted average based on their homogeneity likelihoods $P(s_j|\textbf{x}_j)$~\cite{HoiemIJCV2007,HoiemGeometric2005}, where $\textbf{x}_j$ is the corresponding feature vector. The likelihood of a segment label is then given as:\vspace*{-0.05in}
\[
P(y_i=k|\textbf{x}_i) = \sum\limits_{j}^{n_s} P(y_j = k|\textbf{x}_j,s_j) P(s_j|\textbf{x}_j),
\]
where, $k$ denotes the possible geometric labels and $n_s$ are number of hierarchical segmentations. This technique yields a final classification of super-pixels at the over-segmentation level by combining the individual predictions across hierarchy levels. These weighted posterior probabilities of super-pixels, for main and sub-vertical class, are then averaged across frames in a temporal window to give final predictions for each super-voxel.


==> intro_copy.tex <==

\section{Introduction}
\label{sec:intro}

\noindent Holistic scene understanding requires an understanding of the broad 3D structure of the scene, and the relation of its objects present. One important step towards this goal is to partition a scene into regions and label them relative to each other and within the scene geometry. Geometric classes can define the basic 3D structure of a scene \wrt the camera, \eg whether surfaces are horizontally, supports objects or are vertical \wrt the camera. Early work by Hoeim \etal\cite{hoiem2006putting} showed that geometric context can be used to obtain a probabilistic representation of the scene layout based on geometric classes which in turn can be used to improve object detection. Torralba \etal \cite{torralba2004contextual}, showed that global context plays an important role in object detection. Recently, Divala\etal \cite{empiricalContext}, showed that incorporating geometric context information, not only improves object detection but also makes  misclassifications more reasonable. 

\begin{figure}
\centering
%\vspace{-0.5cm}
\includegraphics[scale=.35, trim=10pt 20pt 20pt 20pt]{fig1_new.pdf}
\setlength\fboxsep{0pt}
\setlength\fboxrule{0.5pt}
\fbox{\includegraphics[scale=.25]{legend.pdf}}
\vspace{-0.05in}
\caption{\small{A video frame of an urban scene (left) and the predicted geometric context of our system (right). We achieve high accuracy leveraging motion and appearance features while achieving temporal consistency by relying on spatio-temporal regions across various granularities. Please watch accompanying video.}}
\vspace{-0.1in}
\label{fig:f1}
\end{figure}

Although progress has been made for scene understanding in the image domain few work has addressed geometric context in videos. Where image based systems aim to label 2D- regions or individual pixels, video generalizes this concept to label spatio-temporal regions that exhibit coherence in motion and appearance. Therefore, as we will empirically demonstrate in \cref{sec:results}, a system for geometric context of video that has been trained on videos is expected to outperform a system that is trained on individual frames. Furthermore, image based systems treat each frame independently, without exploiting temporal causality and redundancy present in video.

In this paper, we propose a method to provide a high level description of a \emph{video} scene by assigning geometric classes to spatio-temporal regions as shown in \cref{fig:f1}. Building upon a hierarchical video-segmentation to achieve temporal consistency, we compute a wide variety of appearance, location, and motion features which are used to train classifiers to predict geometric context in video. A significant challenge for developing scene understanding system for videos is, that to best of our knowledge, there is no completely annotated \emph{video} dataset available for training and evaluation. To overcome this limitation, we have collected and annotated a video dataset with pixel level ground truth labels of for over 20,000 frames across 100 videos covering a wide variety of scene examples. In particular, the contributions of this paper are:
\begin{list}{$\bullet$}
{\setlength{\leftmargin}{1ex}\setlength{\labelsep}{.5ex}\setlength{\parsep}{.4ex plus .2ex minus .1ex}\setlength{\itemsep}{0ex plus .1ex}\setlength{\topsep}{0ex plus .1ex}}
\item A highly accurate scene description for video via geometric classes (96\% accuracy across main geometric classes).
\item Exploiting motion and temporal causality/redundancy present in video by using motion features and aggregating predictions across spatio-temporal regions.
\item A novel dataset of 100 annotated videos ($\sim$20,000 frames) with pixel level labels.
\item Combination of multiple segmentation granularities via homogeneity prediction alleviating the need to determine correct granularity a priori.
\item A semi-supervised bootstrap learning framework for expanding the pool of labeled data with highly confident predictions obtained on unlabeled data.
\end{list}


==> related_copy.tex <==
\section{Related Work}
%*** outline: Need to show that video based system is required, and there is no exising system n dataset for video
%Hoeim’s et al work, and other works, about other existing datasets
%outline contributions n results should follow order //// 

 %*** from Matthias’s video segmentation paper (to motivate video over image comments)  \\
\noindent Image based scene understanding methods~\cite{HoiemIJCV2007,gould2009decomposing} can be directly applied to video frames without considering temporal coherence and can generate a description of the scene. However, these methods lack temporal information from neighboring frames and may result in temporally inconsistent flickering labels across frames. These inconsistent labels can impact performance, i.e., scene labels from one frame can suddenly change in next frame. In addition, such a method would not benefit from spatio-temporal and causal techniques to process videos efficiently, e.g., an image based system would process each segment in video independently, resulting in long processing time. 

%*** talk abt video systems, structure form motion and frame by frame methods\\
Temporal information can be incorporated using structure from motion ~\cite{sturgess2009combining,brostow2008segmentation}, which is slow and may require large buffer \hrnote{ from temporal consistency paper, need to rephrase}. Another approach to achieve temporal consistency across frames is to use optical flow between consecutive frames to estimate the neighborhood of each pixel and then combine past predictions to make final prediction~\cite{miksik-cmutr-12}. This requires labeling every pixel in every frame in the video independently, which doesn't leverage the causality in video. Our video scene understanding approach takes advantage of spatio-temporal information in videos by using hierarchical video segmentation, which segments a video into spatio-temporal regions~\cite{MatthiasSegmentation}. Further, we leverage from causality in videos to efficiently label videos, which is linear to number of unique segments in videos. It is not affected by number of frames, or number of segments per frame, as an image based or independent frame by frame labeling method would. 

%%% do we have a online - steaming video segmentation ?? more suitable for mobile robot ??
%*** end



%***  No Need, after first para : talk about Hoeim et al, image based system, differences??\\
%Hoeim \textit{et. al.}, performed the geometric context labeling on a dataset of three hundred images~\cite{HoiemIJCV2007,HoiemGeometric2005}. They proposed color, texture, location, and perspective features for proposing image labeling method. In addition to these features, we include motion based features, and take advantage of spatio-temporal context and causality to efficiently process videos. 

%% talk about segmentation (not a contribution of this paper)

%*** talk about semi-supervised method\\
A hurdle in video scene understanding has been availability of ground truth annotated dataset. Ground truth annotation is a challenging and time consuming task. To accelerate video scene understanding studies, We have created a ground truth annotated dataset of 100 videos, containing about 20000 frames. To learn from unlabeled data, we propose to use semi-supervised bootstrapping learning in a hierarchical video segmentation.  

%*** summary and contribution \\
\noindent Our video scene analysis method builds on the work of Hoeim \textit{et. al.} image based approach~\cite{HoiemIJCV2007}. We extend image based approach to video by taking advantage of spatio-temporal context, and causality in videos. \hrnote{repeat of intro, to be removed} Following are the main contributions of our work: i) a video scene understanding system, ii) efficient processing of video using causality in videos, iii) showing that temporal and motion based features improve object detection in video scenes, iv) a video dataset with pixel-level annotation of about 20000 frames (100 videos), v) semi-supervised bootstrapping method in hierarchical video segmentation setting to improve scene labeling from unlabeled videos.

%-------------------------------------------------------------------------
